GNNear: Accelerating Full-Batch Training of Graph Neural Networks with Near-Memory Processing

Recently, Graph Neural Networks (GNNs) have become state-of-the-art algorithms for analyzing non-euclidean graph data. However, to realize efficient GNN training is challenging, especially on large graphs. The reasons are many-folded: 1) GNN training incurs a substantial memory footprint. Full-batch training on large graphs even requires hundreds to thousands of gigabytes of memory. 2) GNN training involves both memory-intensive and computation-intensive operations, challenging current CPU/GPU platforms. 3) The irregularity of graphs can result in severe resource under-utilization and load-imbalance problems. This paper presents a GNNear accelerator to tackle these challenges. GNNear adopts a DIMM-based memory system to provide sufficient memory capacity. To match the heterogeneous nature of GNN training, we offload the memory-intensive Reduce operations to in-DIMM Near-Memory-Engines (NMEs), making full use of the high aggregated local bandwidth. We adopt a Centralized-Acceleration-Engine (CAE) to process the computation-intensive Update operations. We further propose several optimization strategies to deal with the irregularity of input graphs and improve GNNear's performance. Comprehensive evaluations on 16 GNN training tasks demonstrate that GNNear achieves 30.8$\times$/2.5$\times$ geomean speedup and 79.6$\times$/7.3$\times$(geomean) higher energy efficiency compared to Xeon E5-2698-v4 CPU and NVIDIA V100 GPU.

==> acmart/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> figtex/fig_distribute_compare.tex <==
\begin{figure} [t]
% \setlength{\abovecaptionskip}{-1pt}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/distribute.pdf} 
      \caption{Comparisons with DistGNN and Roc.}
            \label{fig:dist_compare}
                        % \vspace{-1em}
\end{figure}


==> figtex/fig_imbalance.tex <==
\begin{figure} [h]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/imbalance.pdf} 
                         \vspace{-8pt}
    \caption{Workload-imbalance Issue. }
         \label{fig:imbalance}
        %  \vspace{-1em}
\end{figure}

==> figtex/fig_scalability.tex <==
\begin{figure} [t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/scalability.pdf} 
    \caption{Scalability}  
         \label{fig:scalability}
        %  \vspace{-1em}
\end{figure}


==> figtex/fig_training_flow.tex <==
\begin{figure*} [t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/flow.pdf} 
    \caption{Computation flow of GCN training. \todo{dimension?} \textcircled{\scriptsize{1}}\textcircled{\scriptsize{3}}: Forward aggregation. \textcircled{\scriptsize{2}}\textcircled{\scriptsize{4}}: Forward combination. \textcircled{\scriptsize{5}}: Loss computation.  \textcircled{\scriptsize{6}}\textcircled{\scriptsize{8}}: Feature/weight gradients computation. \textcircled{\scriptsize{7}}\textcircled{\scriptsize{9}}: Feature gradients aggregation.    Operations marked with orange and blue  denote \texttt{Reduce} and \texttt{Update} operations, respectively.}
      \label{fig:flow}
    %   \vspace{-1em}
\end{figure*}


==> tables/buffered_variables.tex <==
\begin{table}[t]
\caption{Buffered Variables During Training}
\label{buffered_variables}
\vspace{-0.5em}
\setlength{\tabcolsep}{1.4mm}{
\resizebox{0.48\textwidth}{!}{
\renewcommand{\arraystretch}{0.7}{
\begin{tabular}{c|l|l|l|ll|ll|l|l}
\toprule
Step                                                          & \multicolumn{1}{c|}{\textcircled{\scriptsize{1}}} & \multicolumn{1}{c|}{\textcircled{\scriptsize{2}}}                                              & \multicolumn{1}{c|}{\textcircled{\scriptsize{3}}}                                                  & \multicolumn{2}{c|}{\textcircled{\scriptsize{4}}}                                                                                                                      & \multicolumn{2}{c|}{\textcircled{\scriptsize{6}}}                                                                                                                      & \multicolumn{1}{c|}{\textcircled{\scriptsize{7}}}                                                 & \multicolumn{1}{c}{\textcircled{\scriptsize{8}}} \\ \midrule
\begin{tabular}[c]{@{}c@{}}Buffered \\ Variables\end{tabular} & $a_v^l$                & \begin{tabular}[c]{@{}l@{}}$a_v^l$\\ $z_v^l$\\ $h_v^{l}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$a_v^l$\\ $z_v^l$\\ $a_v^{l+1}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$a_v^l$\\ $z_v^l$\\ $a_v^{l+1}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$z_v^{l+1}$\\ $h_v^{L}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$a_v^l$\\ $z_v^l$\\ $a_v^{l+1}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\widehat{\delta}_v^{l+1}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$a_v^l$\\ $z_v^l$\\ $\widehat{\delta}_{v}^{l'}$\end{tabular} & $\widehat{\delta}_v^l$             \\ \bottomrule
\end{tabular}}}}
\vspace{-1em}
\end{table}


==> tex/introduction.tex <==
\section{Introduction}
In recent years, 
% The past few years have witnessed the prosperity of deep neural networks (DNNs), which have became the \emph{defacto} cornerstones for many real world applications, such as image classification~\cite{alexnet}\cite{resnet}\cite{densenet}, object detection~\cite{girshick2015fast}\cite{redmon2017yolo9000}, natural language processing~\cite{sutskever2014sequence}, etc.
% Note that conventional DNNs only take euclidean data as input such as images videos and text sequences. However, nowadays there are also great demands for analysing non-euclidean graph data. 
Graph Convolutional Network~(GCN) has emerged as a state-of-the-art algorithm to analyze non-euclidean graph data. 
Given a graph, a GCN model gets the vertex-level representation with several stacked GCN layers. In each layer, all the vertices first aggregate their neighbors' hidden features, then use one or more fully-connected layers to transform the features and produce the outputs. The final layer's features are treated as the vertex-level representations, which can be used on various down-stream tasks, such as  node classification~\cite{Garcia-DuranN17,GibertVB12,semigcn}, point-cloud~\cite{wang2019graph,xu2020grid,qian2021pu,zhai2020multi}, recommendation systems~\cite{ying2018graph,zhao2019intentgc,wu2019session,wang2019kgat,fan2019metapath}, smart traffic~\cite{zhao2019t,ge2019temporal,cui2019traffic}, IC design~\cite{wang2020gcn,mirhoseini2020chip,zhang2019circuit}, physical system simulation~\cite{henrion2017neural}, and chemical prediction~\cite{gilmer2017neural}. 


\input{figtex/fig_trend}

Though various GCN accelerators have been proposed to improve the efficiency of GCN  inference~\cite{hygcn, geng2019awb, blockgnn, liang2020engn, rubik, legognn,gcnx,song2021cambricon},  existing accelerators and GPU/CPU platforms do not easily support GCN training at scale, because GCN training task has three peculiar challenges: (1) GCN training incurs a large memory footprint. To enable back-propagation, we have to buffer a huge amount of intermediate data. According to a previous work's profiling results~\cite{fuseGNN}, even the middle-scale Reddit dataset~\cite{graphSAGE} containing 114 million edges takes up 58 GB memory using PyG-GPU framework~\cite{pyg}, exceeding  most GPUs' capacity. In the meanwhile, as illustrated in Figure~\ref{fig:trend}, we observe that the scale of  graphs applied in GCN researches have been growing exponentially in recent years~\cite{semigcn,graphSAGE,clustergcn,hu2020ogb}.  Though  mini-batch training strategies with neighbor-sampling~\cite{fastgcn,clustergcn,graphSAGE,zeng2019graphsaint} substantially reduce the memory requirement, they are proved to have lower accuracy compared to full-graph training due to approximation errors~\cite{graphSAGE,distgnn,roc,tripathy2020reducing,dgcl}.  (2) GCN training involves both memory-intensive (e.g. 0.5 ops/Byte) feature/gradient reduction operations and  computation-intensive (e.g. 256 ops/Byte) feature/gradient update operations. Neither PIM/NDP-based graph accelerators\cite{zhuo2019graphq,graphp,ahn2015scalable, dai2018graphh} (optimized for memory access)  nor traditional DNN accelerators\cite{chen2014diannao,jouppi2017datacenter,eyeriss, dadiannao, tangram, zhang2015optimizing} (optimized for computation) can well-handle such a discrepancy in GCN training.  (3) The complex GCN training dataflow, along with the irregularity of real-world graphs (e.g., the sparse connectivity and diverse input feature dimensions of graphs), jointly increase the difficulty of optimizing a distributed training system's efficiency. 


To tackle these challenges, we propose \texttt{GCNear}, a novel hybrid GCN training accelerator that harnesses near-memory processing (NMP) technique to achieve high-throughput, energy-efficient, and scalable GCN training. In this paper, we first conduct a detailed analysis of GCN training  and categorize the involved operations as memory-intensive \texttt{Reduce} and computation-intensive \texttt{Update} operations. We then offload \texttt{Reduce} operations to on-DIMM Near-Memory Engines (NMEs). In this way, we  take full advantage of  easy-to-scale memory capacity and high aggregated local bandwidth of DIMM-based memory system to conduct efficient near-memory reduction. For \texttt{Update} operations, we adopt a Centralized ASIC Engine (CAE) to provide sufficient computation capacity. To further improve the performance of such a heterogeneous system and deal with irregular input graphs, we elaborate on the data mapping, data reuse, and  dataflow scheduling strategies, etc. Our comprehensive evaluations on large real-world graphs demonstrate that \texttt{GCNear} has \geomeanSpeedupOverCPU~/~\geomeanSpeedupOverGPU~geomean speedup and \geomeanEnergySavingOverCPU~/ \geomeanEnergySavingOverGPU~higher energy-efficiency (geomean) compared to Xeon E5-2698-v4 CPU and NVIDIA V100 GPU. We also discuss the scalability of \texttt{GCNear} by proposing a Multi-GCNear system to deal with super-large graphs and deep models. Compared to state-of-the-art Roc and DistGNN systems, Multi-GCNear has up to~\SpeedupOverRoc~and~\SpeedupOverDistGNN~higher training speed. 
 To summarize, we make the following contributions:

\begin{itemize}
    \item We analyse the challenges in GCN training  and  categorize the operations as memory-intensive \texttt{Reduce} and computation-intensive \texttt{Update} operations. (Section \ref{sec:heterogeneous})
    \item We propose \texttt{GCNear}, the first hybrid GCN training  accelerator leveraging both DIMM-based NDP engines  and a centralized ASIC engine to provide low-cost and easy-to-scale memory capacity and match the heterogeneous nature of GCN training.  (Section \ref{sec:proposal} )
    \item We propose several optimization strategies  to improve \texttt{GCNear}'s training efficiency. A Multi-GCNear system is also discussed to deal with the emerging super-large graphs  and deep models (Section \ref{sec:optimization}\&\ref{sec:multi})
    % \item We discuss the scalability of \texttt{GCNear} and propose a Multi-GCNear system for training on super-large graphs and deep models (Section~\ref{sec:multi}). 
    \item We conduct extensive experiments on various GCN training tasks and demonstrate the superiority of  \texttt{GCNear} accelerator and Multi-GCN system over commercial CPU/GPU platforms and two state-of-the-art distributed training solutions Roc and DistGNN.  (Section \ref{sec:evaluation}\&\ref{sec:multi})

\end{itemize}

==> todo.tex <==
✅1. Figure-17 有个数据改一下
✅2. Figure-19 有个数据改一下
✅3. Figure-21(d) 数据
4. Simulation methodology 那里改一下描述

